Automated MPI-X code generation for scalable finite-difference solvers

Partial differential equations (PDEs) are crucial in modeling diverse phenomena across scientific disciplines, including seismic and medical imaging, computational fluid dynamics, image processing, and neural networks. Solving these PDEs at scale is an intricate and time-intensive process that demands careful tuning. This paper introduces automated code-generation techniques specifically tailored for distributed memory parallelism (DMP) to execute explicit finite-difference (FD) stencils at scale, a fundamental challenge in numerous scientific applications. These techniques are implemented and integrated into the Devito DSL and compiler framework, a well-established solution for automating the generation of FD solvers based on a high-level symbolic math input. Users benefit from modeling simulations for real-world applications at a high-level symbolic abstraction and effortlessly harnessing HPC-ready distributed-memory parallelism without altering their source code. This results in drastic reductions both in execution time and developer effort. A comprehensive performance evaluation of Devito's DMP via MPI demonstrates highly competitive strong and weak scaling on CPU and GPU clusters, proving its effectiveness and capability to meet the demands of large-scale scientific simulations.

==> mnsc_time_results.tex <==

\begin{figure*}[!htbp]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_runtime_so-04.pdf}
        \caption{SDO 4}
        \label{fig:ac_so04_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_runtime_so-08.pdf}
        \caption{SDO 8}
        \label{fig:ac_so08_runtime}
    \end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_runtime_so-12.pdf}
        \caption{SDO 12}
        \label{fig:ac_so12_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_runtime_so-16.pdf}
        \caption{SDO 16}
        \label{fig:ac_so16_runtime}
	\end{subfigure}
        \caption{Multi-node execution time strong scaling of the \textbf{isotropic acoustic}
        stencil kernel for varying space orders (4, 8, 12, 16) on a $1024^3$ computational domain
        with 293 timesteps (Lower values indicate better performance).}
    \label{fig:ac-stencil-scaling-runtime}
\end{figure*}


\begin{figure*}[!htbp]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_runtime_so-04.pdf}
        \caption{SDO 4}
        \label{fig:el_so04_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_runtime_so-08.pdf}
        \caption{SDO 8}
        \label{fig:el_so08_runtime}
    \end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_runtime_so-12.pdf}
        \caption{SDO 12}
        \label{fig:el_so12_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_runtime_so-16.pdf}
        \caption{SDO 16}
        \label{fig:el_so16_runtime}
	\end{subfigure}
        \caption{Multi-node execution time strong scaling of the \textbf{isotropic elastic}
        stencil kernel for varying space orders (4, 8, 12, 16) on a $1024^3$ computational domain
        with 290 timesteps (Lower values indicate better performance).}
        \label{fig:el-stencil-scaling-runtime}
\end{figure*}

\begin{figure*}[!htbp]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_runtime_so-04.pdf}
        \caption{SDO 4}
        \label{fig:tti_so04_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_runtime_so-08.pdf}
        \caption{SDO 8}
        \label{fig:tti_so08_runtime}
    \end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_runtime_so-12.pdf}
        \caption{SDO 12}
        \label{fig:tti_so12_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_runtime_so-16.pdf}
        \caption{SDO 16}
        \label{fig:tti_so16_runtime}
	\end{subfigure}
        \caption{Multi-node execution time strong scaling of the \textbf{anisotropic acoustic (TTI)}
        stencil kernel for varying space orders (4, 8, 12, 16) on a $1024^3$ computational domain
        with 290 timesteps (Lower values indicate better performance).}
    \label{fig:tti-stencil-scaling-runtime}
\end{figure*}


==> snsc_time_results.tex <==
\begin{figure*}[!htbp]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_SN_runtime_so-04.pdf}
        \caption{SDO 4}
        \label{fig:ac_sn_so04_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_SN_runtime_so-08.pdf}
        \caption{SDO 8}
        \label{fig:ac_sn_so08_runtime}
    \end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_SN_runtime_so-12.pdf}
        \caption{SDO 12}
        \label{fig:ac_sn_so12_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_SN_runtime_so-16.pdf}
        \caption{SDO 16}
        \label{fig:ac_sn_so16_runtime}
	\end{subfigure}
        \caption{Execution time throughput strong scaling of the \textbf{isotropic acoustic}
        stencil kernel for varying space orders (4, 8, 12, 16) on a $1024^3$ computational domain
        with 290 timesteps (Lower values indicate better performance).}
        \label{fig:ac-sn-stencil-scaling-runtime}
\end{figure*}

\begin{figure*}[!htbp]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_SN_runtime_so-04.pdf}
        \caption{SDO 4}
        \label{fig:el_sn_so04_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_SN_runtime_so-08.pdf}
        \caption{SDO 8}
        \label{fig:el_sn_so08_runtime}
    \end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_SN_runtime_so-12.pdf}
        \caption{SDO 12}
        \label{fig:el_sn_so12_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_SN_runtime_so-16.pdf}
        \caption{SDO 16}
        \label{fig:el_sn_so16_runtime}
	\end{subfigure}
        \caption{Execution time strong scaling of the \textbf{isotropic elastic}
        stencil kernel for varying space orders (4, 8, 12, 16) on a $1024^3$ computational domain
        with 363 timesteps (Lower values indicate better performance).}
        \label{fig:el-sn-stencil-scaling-runtime}
\end{figure*}

\begin{figure*}[!htbp]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_SN_runtime_so-04.pdf}
        \caption{SDO 4}
        \label{fig:tti_sn_so04_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_SN_runtime_so-08.pdf}
        \caption{SDO 8}
        \label{fig:tti_sn_so08_runtime}
    \end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_SN_runtime_so-12.pdf}
        \caption{SDO 12}
        \label{fig:tti_sn_so12_runtime}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_SN_runtime_so-16.pdf}
        \caption{SDO 16}
        \label{fig:tti_sn_so16_runtime}
	\end{subfigure}
        \caption{Execution time strong scaling of the \textbf{anisotropic acoustic (TTI)}
        stencil kernel for varying space orders (4, 8, 12, 16) on a $1024^3$ computational domain
        with 290 timesteps (Lower values indicate better performance).}
    \label{fig:tti-sn-stencil-scaling-runtime}
\end{figure*}


==> trash.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/mpi-basic.pdf}
    \caption{Basic mode}
    \label{fig:mpi-basic}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/mpi-diag2.pdf}
    \caption{Diagonal mode}
    \label{fig:mpi-diag2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/mpi-full.pdf}
    \caption{Full mode}
    \label{fig:mpi-full}
    \end{subfigure}
    \caption{Schematic representation of the available MPI modes.}
    \label{fig:mpi-modes}
\end{figure*}

\begin{figure*}[h]
\centering
\begin{ganttchart}[
            x unit=0.7cm,
            y unit chart=0.7cm,
            canvas/.style={draw=none,fill=none}, %
            vgrid={*1{draw=black!12}},           %
            inline,                              %
            group/.style={draw=none,fill=none},  %
            bar top shift=0.1,                   %
            bar height=0.8,                      %
            y unit title=0.5cm,                  %
            title/.style={draw=none,fill=none},  %
            include title in canvas=false        %
    ]{-1}{12}


    \ganttgroup[inline=false]{$Basic$}{0}{1}
    \ganttbar[bar/.style={fill=yellow}]{$haloupdate$}{0}{2}
    \ganttbar[bar/.style={fill=orange}]{$compute$}{3}{5}\\

    \ganttgroup[inline=false]{$Diagonal$}{0}{1}

    \ganttbar[bar/.style={fill=yellow}]{$compute$}{0}{2}
    \ganttbar[bar/.style={fill=yellow}]{$halowait$}{0}{2}
    \ganttbar[bar/.style={fill=yellow}]{$remainder$}{0}{2}\\

    \ganttgroup[inline=false]{$Full$}{0}{1}
    
\end{ganttchart}
\caption{A schematic example of the communication and computation phases for each timestep}
\label{fig:schedule}
\end{figure*}


\begin{figure*}[ht]
\centering
\centering
\begin{subfigure}[b]{\textwidth}
\begin{tikzpicture}[
    node distance=5cm, %
    block/.style={rectangle, draw, text width=2cm, align=left, minimum height=.5cm},
    redbox/.style={block, fill=red!30},
    redgreenbox/.style={block, fill=green!30},
    bluebox/.style={block, fill=blue!30},
    arrow/.style={thick,-stealth}
    ]
    \node[redbox] (haloupdate) {haloupdate};
    \node[redgreenbox, right of=haloupdate] (compute) {compute};
    
    \draw[arrow] (haloupdate) -- (compute);
\end{tikzpicture}
\caption{Basic mode}
\label{fig:pipe-basic}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\begin{tikzpicture}[
    node distance=3.5cm, %
    block/.style={rectangle, draw, text width=2cm, align=left, minimum height=.5cm},
    redbox/.style={block, fill=red!30},
    greenbox/.style={block, fill=green!30},
    bluebox/.style={block, fill=blue!30},
    arrow/.style={thick,-stealth}
    ]
    \node[redbox] (haloupdate) {haloupdate};
    \node[bluebox, right of=haloupdate] (halowait) {halowait};
    \node[greenbox, right of=halowait] (compute) {compute};
    
    \draw[arrow] (haloupdate) -- (halowait);
    \draw[arrow] (halowait) -- (compute);
\end{tikzpicture}
\caption{Diagonal mode}
\label{fig:pipe-diag2}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\begin{tikzpicture}[
    node distance=3.5cm, %
    block/.style={rectangle, draw, text width=2cm, align=left, minimum height=.5cm},
    redbox/.style={block, fill=red!30},
    greenbox/.style={block, fill=green!30},
    bluebox/.style={block, fill=blue!30},
    arrow/.style={thick,-stealth}
    ]
    \node[redbox] (haloupdate) {haloupdate};
    \node[bluebox, right of=haloupdate] (halowait) {halowait};
    \node[greenbox, right of=halowait] (compute) {compute};
    
    \draw[arrow] (haloupdate) -- (halowait);
    \draw[arrow] (halowait) -- (compute);
\end{tikzpicture}
\caption{Full mode}
\label{fig:pipe-full}
\end{subfigure}
\caption{Overview of the MPI modes pipeline}
\label{fig:pipe-fdiag2}
\end{figure*}




\begin{table}[!htbp]
    \centering
    \begin{threeparttable}[c]
    \begin{tabular}{|p{1.2cm}|p{1.2cm}|p{1.1cm}|p{1.1cm}|p{1.1cm}|  }
    \hline
    \multicolumn{5}{|c|}{Computational properties per stencil kernel} \\
    \hline
                            & SDO$^{a}$
                            & Unopt
                            & Opt
                            & OI$^{b}$\\
                            \hline
    \rotatebox{0}{Acoustic} &  4  &   104  &   34 &  1.93  \\  \cline{2-5}
                            &  8  &   128  &   48 &  2.64  \\  \cline{2-5}
                            & 12  &   152  &   62 &  3.28  \\  \cline{2-5}
                            & 16  &   176  &   76 &  3.85  \\  \hline
    \rotatebox{0}{Elastic}  &  4  &   432  &  165 &  1.88  \\  \cline{2-5}
                            &  8  &   648  &  269 &  2.99  \\  \cline{2-5}
                            & 12  &   864  &  373 &  4.03  \\  \cline{2-5}
                            & 16  &  1080  &  477 &  5.02  \\  \hline
    \rotatebox{0}{TTI}      &  4  &   824  &  104 &  2.17  \\  \cline{2-5}
                            &  8  &  2080  &  166 &  4.37  \\  \cline{2-5}
                            & 12  &  3912  &  225 &  6.91  \\  \cline{2-5}
                            & 16  &  6320  &  284 & 10.09  \\  \hline
           
    \end{tabular}
    \caption{Floating point operations and operational intensity for the evaluated stencil kernels}
    \label{table:flops_table}
    \begin{tablenotes}[flushleft]
    \item [a] Space discretisation order
    \item [b] Operational Intensity
    \end{tablenotes}
    \end{threeparttable}
    \end{table}
    




    \subsubsection{Single-node multi-socket - strong scaling results}\label{sec:results:single-node-multi-socket}

The evaluated architecture is highly interesting for single-node multi-socket
experiments due to its NUMA architecture. It is recommended to use one MPI
process per NUMA region (i.e. at least 8 MPI processes per node) and 16 OpenMP
threads running at the same NUMA region as their parent MPI process.
DMP is mainly employed to decompose problems so that they fit in a single node,
however, another benefit of DMP is to reducing data movement and enhance locality
when it comes for architectures with several NUMA nodes.

Figures \ref{fig:ac-stencil-singlenode-scaling}, \ref{fig:el-stencil-singlenode-scaling},
\ref{fig:tti-stencil-singlenode-scaling} demonstrate the single-node multi-socket throughput
achieved for the AMD EPYC7742 detailed in \autoref{sec:cpu-overall}, for the isotropic
acoustic, isotropic elastic and TTI respectively.
Bars show the achieved Gpts/s for every benchmark while the \emph{ideal scaling}
line shows the possible ideal achieved performance based upon the best performance
of the first set of bars. This is the best Gpts/s for the single-socket execution
for the single-node performance (intra-node strong scaling) and the best Gpts/s
for the single-node execution for the multi-node strong scaling performance (inter-node strong scaling).

Each set of subfigures showcases the results for varying space discretization orders.

The isotropic acoustic performs better with \emph{basic} and \emph{full} mode
and exhibits around 90\% to 80\% efficient scaling intra-node as we move to
higher space orders.
The isotropic elastic performs better with \emph{diag2} and \emph{full} mode
exhibiting $\approx 50\text{-}60\%$ efficiency.
\emph{basic} and \emph{diag2} modes benefit mostly the anisotropic acoustic (TTI)
kernels exhibiting around $\approx 55\text{-}65\%$ intra-node scaling efficiency.


\begin{figure*}[!htbp]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_SN_throughput_so-04.pdf}
        \caption{SDO 4}
        \label{fig:ac_sn_so04_platform}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_SN_throughput_so-08.pdf}
        \caption{SDO 8}
        \label{fig:ac_sn_so08_platform}
        \end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_SN_throughput_so-12.pdf}
        \caption{SDO 12}
        \label{fig:ac_sn_so12_platform}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Acoustic_SN_throughput_so-16.pdf}
        \caption{SDO 16}
        \label{fig:ac_sn_so16_platform}
	\end{subfigure}
        \caption{Throughput strong scaling of the \textbf{isotropic acoustic} stencil kernel
        for varying space orders (4, 8, 12, 16) on a $1024^3$ computational domain
        with 293 timesteps (Higher values indicate better performance).}
    \label{fig:ac-stencil-singlenode-scaling}
\end{figure*}

\begin{figure*}[!htbp]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_SN_throughput_so-04.pdf}
        \caption{SDO 4}
        \label{fig:el_sn_so04_platform}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_SN_throughput_so-08.pdf}
        \caption{SDO 8}
        \label{fig:el_sn_so08_platform}
    \end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_SN_throughput_so-12.pdf}
        \caption{SDO 12}
        \label{fig:el_sn_so12_platform}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/Elastic_SN_throughput_so-16.pdf}
        \caption{SDO 16}
        \label{fig:el_sn_so16_platform}
	\end{subfigure}
        \caption{Throughput strong scaling of the \textbf{isotropic elastic} stencil kernel
        for varying space orders (4, 8, 12, 16) on a $1024^3$ computational domain
        with 363 timesteps (Higher values indicate better performance).}
    \label{fig:el-stencil-singlenode-scaling}
\end{figure*}

\begin{figure*}[!htbp]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_SN_throughput_so-04.pdf}
        \caption{SDO 4}
        \label{fig:tti_sn_so04_platform}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_SN_throughput_so-08.pdf}
        \caption{SDO 8}
        \label{fig:tti_sn_so08_platform}
    \end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_SN_throughput_so-12.pdf}
        \caption{SDO 12}
        \label{fig:tti_sn_so12_platform}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/TTI_SN_throughput_so-16.pdf}
        \caption{SDO 16}
        \label{fig:tti_sn_so16_platform}
	\end{subfigure}
        \caption{Throughput strong scaling of the \textbf{anisotropic acoustic (TTI)}
        stencil kernel for varying space orders (4, 8, 12, 16) on a $1024^3$
        computational domain with 293 timesteps (Higher values indicate better performance).}
    \label{fig:tti-stencil-singlenode-scaling}
\end{figure*}




\begin{table}[!htbp]
    \centering
    \begin{threeparttable}[c]
    \begin{tabular}{|p{1.2cm}|p{1.2cm}|p{1.3cm}|p{1.4cm}|  }
    \hline
    \multicolumn{4}{|c|}{Full percentages} \\
    \hline
                            & SO/NN
                            & 1
                            & 128 \\
                            \hline
    \rotatebox{0}{Acoustic} &  4  & 93/5/0/0  &   34          \\  \cline{2-4}
                            &  8  & 87/10/2/2 &   48          \\  \cline{2-4}
                            & 12  & 80/15/2/2 &   62          \\  \cline{2-4}
                            & 16  & 75/20/2/2 &  55/31/10/3   \\  \hline
    \rotatebox{0}{Elastic}  &  4  &   432     &  165          \\  \cline{2-4}
                            &  8  &   648     &  269          \\  \cline{2-4}
                            & 12  &   864     &  373          \\  \cline{2-4}
                            & 16  &  1080     &  477          \\  \hline
    \rotatebox{0}{TTI}      &  4  &   824     &  104          \\  \cline{2-4}
                            &  8  &  2080     &  166          \\  \cline{2-4}
                            & 12  &  3912     &  225          \\  \cline{2-4}
                            & 16  &  6320     &  284          \\  \hline
            
    \end{tabular}
    \caption{Percentages in \emph{full}, drop or remake in smarter way}
    \label{table:flops_table}
    \end{threeparttable}
    \end{table}
    



use the symbol $\bot$ on the LHS and incorporate a \HaloTouch object on the RHS to signify halo accesses (see \autoref{lst:comms}).

 These expressions contain metadata specifying where data communications and halo exchanges should take place and are propagated to the IET level to facilitate halo exchange generation.
    
    \begin{python}[label=lst:comms, caption={The $\bot$ symbol expression with a \HaloTouch on its RHS
            denotes a mock expression for a halo exchange.
            Its iteration space consists of time only, denoting a possible halo exchange for every timestep
            before iterating over the spatial dimensions of the FD grid.}]
    > p clusters
    [Cluster([Eq(u[t1, x + 2, y + 2], ...)])]        
    
    ---> clusters = Communications().process(clusters)
    
    > p clusters
    [Cluster([Eq(|$ \bot $|, HaloTouch(u))]),
     Cluster([Eq(u[t1, x + 2, y + 2], ...)])]
    
    > clusters[0].ispace
    IterationSpace[time[0,0]<336>++]
    
    > clusters[1].ispace        
    IterationSpace[time[0,0]<336>++, x[0,0]<336>++,
                    y[0,0]<336>++]
    \end{python}

